Plan Arithmetic: Compositional Plan Vectors for Multi-Task Control

Autonomous agents situated in real-world environments must be able to master large repertoires of skills. While a single short skill can be learned quickly, it would be impractical to learn every task independently. Instead, the agent should share knowledge across behaviors such that each task can be learned efficiently, and such that the resulting model can generalize to new tasks, especially ones that are compositions or subsets of tasks seen previously. A policy conditioned on a goal or demonstration has the potential to share knowledge between tasks if it sees enough diversity of inputs. However, these methods may not generalize to a more complex task at test time. We introduce compositional plan vectors (CPVs) to enable a policy to perform compositions of tasks without additional supervision. CPVs represent trajectories as the sum of the subtasks within them. We show that CPVs can be learned within a one-shot imitation learning framework without any additional supervision or information about task hierarchy, and enable a demonstration-conditioned policy to generalize to tasks that sequence twice as many skills as the tasks seen during training. Analogously to embeddings such as word2vec in NLP, CPVs can also support simple arithmetic operations -- for example, we can add the CPVs for two different tasks to command an agent to compose both tasks, without any additional training.

==> tableNN.tex <==
\begin{table}[h]
\caption{Each model was trained on tasks contained up to four skills. A task could use the same skill 4 times rather than 4 different skills. We evaluate the models on 40 tasks with 4 skills, 40 tasks with 8 skills, and 40 compositions of two 4 skill tasks. The $D$ column indicates the embedding dimension,  the S column indicates the success rate (higher is better), and the T column indicates the average number of steps until success (lower is better). In S columns we bold the must successful models, and in the T column we bold the most efficient of the most successful models. The CPV model is both the most successful and efficient. For each model we list the success rate of the best epoch of training. All numbers are averaged over 40 trajectories.}
\label{tab:eval}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{lc|cc|cc|cc}
\toprule
Model & $D$ & \multicolumn{2}{|c|}{4 Skills} & \multicolumn{2}{|c|}{8 Skills} & \multicolumn{2}{|c}{$4+4$ Skills}  \\
\midrule
&&S&T&S&T&S&T\\
\midrule

TECNet    & 128 & \\
TECNet    & 256 & 0.85 & 312& 0.57 & 686 &  0.55 &516\\
TECNet    & 512 & 0.75 & 432 & 0.45 & 421 & 0.37 & 969\\
CPV       & 64  & 0.97 & 169 & 0.87 & 260& 0.65 & 433\\
CPV       & 128 & 0.92 & 223 & 0.82 & 298 & 0.50 & 473\\
CPV       & 256 & \textbf{1.0} & \textbf{191}& 0.9 & 326 & 0.62 &434\\
CPV       & 512 & 0.97 & 146& \textbf{0.92} & \textbf{292} & \textbf{0.70} & \textbf{404}\\
\midrule
Expert &  & 1.0 & 53 & 1.0 & 92 & 1.0 & 92 \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table}

